Deep Probability Estimation

Reliable probability estimation is of crucial importance in many real-world applications where there is inherent (aleatoric) uncertainty. Probability-estimation models are trained on observed outcomes (e.g. whether it has rained or not, or whether a patient has died or not), because the ground-truth probabilities of the events of interest are typically unknown. The problem is therefore analogous to binary classification, with the difference that the objective is to estimate probabilities rather than predicting the specific outcome. This work investigates probability estimation from high-dimensional data using deep neural networks. There exist several methods to improve the probabilities generated by these models but they mostly focus on model (epistemic) uncertainty. For problems with inherent uncertainty, it is challenging to evaluate performance without access to ground-truth probabilities. To address this, we build a synthetic dataset to study and compare different computable metrics. We evaluate existing methods on the synthetic data as well as on three real-world probability estimation tasks, all of which involve inherent uncertainty: precipitation forecasting from radar images, predicting cancer patient survival from histopathology images, and predicting car crashes from dashcam videos. We also give a theoretical analysis of a model for high-dimensional probability estimation which reproduces several of the phenomena evinced in our experiments. Finally, we propose a new method for probability estimation using neural networks, which modifies the training process to promote output probabilities that are consistent with empirical probabilities computed from the data. The method outperforms existing approaches on most metrics on the simulated as well as real-world data.

==> csvs/weather_csv.tex <==
Name,Error,ECE,MCE,Loss,Brier,KS Error
CE,33.3667,0.1091,0.2550,0.5997,0.2057,0.1103
Temperature,33.3667,0.0866,0.2356,0.5877,0.2021,0.0741
Platt Regression,31.2333,0.0697,0.1647,0.5738,0.1953,0.0326
Dirichlet,31.2333,0.0697,0.1647,0.5738,0.1953,0.0326
MixNMatch,33.3667,0.0865,0.2358,0.5877,0.2021,0.0739
focal,30.1333,0.0832,0.2125,0.5901,0.2027,0.0445
entropy,32.1333,0.1053,0.2072,0.5783,0.1977,0.0500
MMCE,32.3333,0.0846,0.1973,0.5925,0.2012,0.0731
Deep Ensemble,30.6333,0.0741,0.1824,0.5528,0.1882,0.0757
ours (Binning),29.9667,0.0516,0.1509,0.5425,0.1837,0.0234
ours(KDE) ,30.0667,0.0508,0.1328,0.5432,0.1839,0.0234
